Port-Hamiltonian Architectural Bias for Long-Range Propagation in Deep Graph Networks

The dynamics of information diffusion within graphs is a critical open issue that heavily influences graph representation learning, especially when considering long-range propagation. This calls for principled approaches that control and regulate the degree of propagation and dissipation of information throughout the neural flow. Motivated by this, we introduce (port-)Hamiltonian Deep Graph Networks, a novel framework that models neural information flow in graphs by building on the laws of conservation of Hamiltonian dynamical systems. We reconcile under a single theoretical and practical framework both non-dissipative long-range propagation and non-conservative behaviors, introducing tools from mechanical systems to gauge the equilibrium between the two components. Our approach can be applied to general message-passing architectures, and it provides theoretical guarantees on information conservation in time. Empirical results prove the effectiveness of our port-Hamiltonian scheme in pushing simple graph convolutional architectures to state-of-the-art performance in long-range benchmarks.

==> sections/old.tex <==
\section{Introduction}
Machine learning on graphs gained much attention over the last years due to the general advent of neural networks and the natural occurrence of network-structured data. Similar to convolutional neural networks for images, graph neural networks apply the locality assumption to nodes and their surrounding neighbors. 
A broad variety of methodologies have been proposed to enable information-rich representations of nodes, edges, and graphs to be employed for generative and discriminative models. Eventually, being exploited in drug discovery, recommender systems, or spatiotemporal forecasting \citep{BACCIU2020203}

Irregular graph distributions and the exponential nature of graphs introduce challenges for inductive models to generalize well to unseen examples, especially when the locality assumption is violated and long-range interactions of nodes are of central focus \citep{li2018deeper,zheng2022graph,Pei2020Geom-GCN,platonov2023a,dwivedi2022long}.
\textit{Under-reaching} takes place, when the number of layers does not suffice to connect the information exchange between two nodes to solve the task. With an increasing number of layers, the number of nodes in each node's receptive field grows exponentially. This leads to \textit{over-squashing} of information in the since the embeddings are of fixed dimension \citep{alon2020bottleneck}.
In addition to over-squashing, \cite{li2018deeper} observed that stacking more and more layers is smoothing out the feature representations until no difference between node embeddings can be measured. \cite{di2023understanding} and \cite{RBM23_1054} capture this behavior of \textit{over-smoothing} in terms of a decreasing energy functional of the node embeddings. On the opposite side, \textit{over-sharpening} refers to the case where each node gets such a different embedding, that no patterns can be exploited \citep{di2023understanding}. 
Hence, recent efforts in literature have been devoted to studying the theoretical properties of graph neural networks to guide novel architectures. This thesis follows the line of research interpreting neural networks with residual connections as a numerical integration of a neural-parameterized differential equation, so-called neural ODEs \citep{haber2017stable,chen2018neural}. Utilizing the well-developed tools from dynamical system theory, the forward and backward process of graph neural networks can be analyzed and biased towards favorable properties \citep{eliasof2021pde,gravina2023adgn}.

Hamiltonian dynamics, on the other hand, is a fundamental reformulation of the Newtonian and Lagrangian mechanics in physics which are capable of describing simple systems of springs or pendulums but also complex multi-particle systems \citep{Hairer2006-ks}. By enforcing energy conservation on the system state, the Hamiltonian equations of motion guide the trajectories through space and time. Building on the Lagrangian formulation, Noether stated her fundamental theorem about the inherent connection between symmetries and conservation laws, which will also be the underlying principle in this work \citep{meyer2017introduction}. Besides classical mechanics, these systems are at the core of quantum theory \citep{eisberg1985quantum} and find applications ranging from game theory \citep{GRIFFIN2022127281} to network theory, modeling the information flow in discrete cell automatons \citep{oono1988study,maschke1992intrinsic}.

\section{Hamiltonian Architectures for Deep Graph Neural Networks}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{figures/hamiltoniandgn_v2.pdf}
    \caption{Hamiltonian Deep Graph Network (HDGN). Coupling of two DGNs operating on $\mathbf{p}$ and $\mathbf{q}$ respectively. The gray part shows the energy correction term accounting for the neighbors of the neighbors.}
    \label{fig:HDGN}
\end{figure}
\paragraph{Autonomous Hamiltonian Graph-Coupled Neural ODEs}
\begin{equation}
    \mathbf{y}(0) 
      = \begin{pmatrix}
            \mathbf{p}\\
            \mathbf{q}
        \end{pmatrix} \in \mathbb{R}^{2nd},
        \text{with } \xk
      = \begin{pmatrix}
            \mathbf{p}_k\\
            \mathbf{q}_k
        \end{pmatrix}  \in \mathbb{R}^{2d}
\end{equation}

\begin{align}
\label{eq:HG_vectorized}
        H_{\mathcal{G}}: \mathbb{R}^{2nd} \rightarrow \mathbb{R}, \; \mathbf{y} \rightarrow &\sum_{u \in \mathcal{V}}{\Tilde{\sigma}(\mathbf{W}\xk + \Phi_{\mathcal{G}}(\mathbf{y},\mathcal{N}_u ) + \mathbf{b})^{\top}\mathbf{1}_d}
\end{align}

Having defined this generalized system state, we can define the Hamiltonian dynamics as:

\begin{equation}\label{eq:globalHamilFinal}
    \odv{\mathbf{y}(t)}{t} = \Jskew\nabla_\mathbf{y} H_{\mathcal{G}}(\mathbf{y}(t)) \Leftrightarrow \odv{\mathbf{p}(t)}{t} = -\nabla_{\mathbf{q}} H_{\mathcal{G}}(\mathbf{y}(t)) , \odv{\mathbf{q}(t)}{t} = \nabla_{\mathbf{p}} H_{\mathcal{G}}(\mathbf{y}(t))
\end{equation}
\begin{equation}\label{eq:H_constant}
    \odv{H(\mathbf{y}(t))}{t} = {\pdv{H(\mathbf{y}(t))}{\mathbf{y}(t)}}\cdot\odv{\mathbf{y}(t)}{t} = {\pdv{H(\mathbf{y}(t))}{\mathbf{y}(t)}}\cdot\Jskew\nabla_{\mathbf{y}}H(\mathbf{y}(t)) = 0,
\end{equation}
Inserting our global Hamiltonian \eqref{eq:HG_vectorized} leads to a node-wise dynamic (with $\Jkskew \coloneqq \Lu\Jskew$):
\begin{align}\label{eq:local_dyn}
    \begin{split}
\dxdt = \Jkskew \Lu \dHdy &=\Jkskew(\mathbf{W}^{\top}\sigma(\mathbf{W}\xk(t) + \Phi_{\mathcal{G}}(\mathbf{y}(t),\mathcal{N}_k ) + \mathbf{b})\\&+\sum_{v \in \mathcal{N}_u\cup \{u\}}{\pdv{\Phi_{\mathcal{G}}(\mathbf{y}(t),\mathcal{N}_v )}{\xk(t)}\sigma(\mathbf{W}\xh(t) + \Phi_{\mathcal{G}}(\mathbf{y}(t),\mathcal{N}_v ) + \mathbf{b})})
    \end{split}
\end{align}
Note that we derived a similar statement as \cite{oono1988study}, that the conservation of the order parameter implies the local sum rule: when there is an exchange of order parameter values between a cell and its neighboring cells, there should not be a net change of the order parameter inside the neighborhood surrounding the center cell.
%\begin{lemma}(\cite{Hairer2006-ks}, Theorem 3.3)
%    The so-called symplectic Euler method
%    \begin{equation}
%        \mathbf{p}_{n+1} = \mathbf{p}_n - h\pdv{H_{\mathcal{G}}}{\mathbf{q}}(\mathbf{p}_{n+1},\mathbf{q}_n),\;\;\; \mathbf{q}_{n+1} = \mathbf{q}_n + h\pdv{H_{\mathcal{G}}}{\mathbf{p}}(\mathbf{p}_{n+1},\mathbf{q}_n)
%    \end{equation}
%    and its adjoint method
%     \begin{equation}
%        \mathbf{p}_{n+1} = \mathbf{p}_n - h\pdv{H_{\mathcal{G}}}{\mathbf{q}}(\mathbf{p}_{n},\mathbf{q}_{n+1}),\;\;\; \mathbf{q}_{n+1} = \mathbf{q}_n + h\pdv{H_{\mathcal{G}}}{\mathbf{p}}(\mathbf{p}_{n},\mathbf{q}_{n+1})
%    \end{equation}
%are a symplectic method of order 1.
%\end{lemma}

Inspired by the Hamiltonian ResNet \citep{galimberti2023hamiltonian}, structure assumptions on $\mathbf{W}$ and $\mathbf{V}$ for $\Phi_{\mathcal{G}}((\mathbf{p}_{n+1},\mathbf{q}_n),\mathcal{N}) \coloneqq \sum_{i \in \mathcal{N}}{\mathbf{V}\begin{pmatrix}
    \mathbf{p}_{n+1, i}\\\mathbf{q}_{n,i}
\end{pmatrix}}$, namely $\mathbf{W} = \begin{pmatrix}
    \mathbf{W}_p & \mathbf{0}\\\mathbf{0} & \mathbf{W}_q
\end{pmatrix}$ and $\mathbf{V} = \begin{pmatrix}
    \mathbf{V}_p & \mathbf{0}\\\mathbf{0} & \mathbf{V}_q
\end{pmatrix}$
lead to explicit numerical equations (Semi-implicit Euler)
\begin{align}\label{eq:discretized_local_hamil}\begin{split}
        &\begin{multlined}[c][\linewidth]\mathbf{p}^{(n+1)}_v = 
            \mathbf{p}^{(n)}_v - \epsilon \Biggl[\mathbf{W}_q^{\top}\sigma(\mathbf{W}_q\mathbf{q}^{(n)}_v + \Phi_{\mathcal{G}}(\mathbf{q}^{(n)},\mathcal{N}_v ) + \mathbf{b}_q) \\ - \sum_{u \in \mathcal{N}_v\setminus \{v\}}{\mathbf{V}_q^{\top}}\sigma(\mathbf{W}_q\mathbf{q}^{(n)}_u + \Phi_{\mathcal{G}}(\mathbf{q}^{(n)},\mathcal{N}_u ) + \mathbf{b}_q)\Biggr]\end{multlined}\\
        &\begin{multlined}[c][\linewidth]\mathbf{q}^{(n+1)}_v = \mathbf{q}^{(n)}_v + \epsilon\Biggl[ \mathbf{W}_p^{\top}\sigma(\mathbf{W}_p\mathbf{p}^{(n+1)}_v + \Phi_{\mathcal{G}}(\mathbf{p}^{(n+1)},\mathcal{N}_v ) + \mathbf{b}_p)\\ + \sum_{u \in \mathcal{N}_v\setminus \{v\}}{\mathbf{V}_p^{\top}}\sigma(\mathbf{W}_p\mathbf{p}^{(n+1)}_u + \Phi_{\mathcal{G}}(\mathbf{p}^{(n+1)},\mathcal{N}_u ) + \mathbf{b}_p)\Biggr]\end{multlined}
        \end{split}
\end{align}
\paragraph{Port-Hamiltonian Approach}
Inspired from \cite{desai2021port} we design the dynamics as state-dependent internal dampening and time- and state-dependent external forcing written in terms of the single nodes:
\begin{equation}
    \odv{\mathbf{h}_v(t)}{t} = \left(\Jkskew-\begin{bmatrix}
    D_v(\mathbf{q}) & \mathbf{0}\\\mathbf{0} & \mathbf{0} 
\end{bmatrix} \right)\nabla_{\mathbf{h}_v} H_{\mathcal{G}}(\mathbf{y}) + \begin{bmatrix}
    F_v(\mathbf{q},t)\\\mathbf{0}
\end{bmatrix},\quad \forall k \in \mathcal{V}
\end{equation}
Which can be turned into an adjoint semi-implicit integration scheme:
\begin{align}\label{eq:discrete_portHamil}
    \begin{split}
        \mathbf{q}_v^{(n+1)} &= \mathbf{q}_v^{(n)} + \epsilon\nabla_{\mathbf{p}_v}{{H}_{\mathcal{G}}}(\mathbf{p}^{(n)},\mathbf{q}^{(n+1)}) \\[0.2cm]
    \mathbf{p}_v^{(n+1)} &= \begin{multlined}[t][0.6\textwidth]\mathbf{p}_v^{(n)} + \epsilon\Biggl[\nabla_{\mathbf{q}_v}{{H}_{\mathcal{G}}}(\mathbf{p}^{(n)},\mathbf{q}^{(n+1)}) \\+ D_v(\mathbf{q}^{(n+1)}) \nabla_{\mathbf{p}_v}{{H}_{\mathcal{G}}}(\mathbf{p}^{(n)},\mathbf{q}^{(n+1)}) + F_v(\mathbf{q}^{(n+1)},t)\Biggr]\end{multlined}
    \end{split}
\end{align}

Using this framework, we can understand layer-dependent weights when stacking GNNs, since the weights depend now explicitly on time, i.e., $\mathbf{W}(t)$ and $\mathbf{V}(t)$ which leads to time-varying Hamiltonian functional.
\paragraph{Stability Analysis}
\begin{theorem}[Eigenvalues of the Jacobian]\label{lemma:eigenvaluesJacobian}
The local dynamics \eqref{eq:local_dyn} possess an Jacobian with eigenvalues purely on the imaginary axis, i.e. $$\operatorname{Re}\left(\lambda_i\left(\pdv{}{\mathbf{h}_v}\Jkskew\nabla_{\mathbf{h}_v}H_{\mathcal{G}}(\mathbf{y}(t))\right)\right) = 0\quad ,\forall i$$
\end{theorem}

\begin{lemma}[Divergence-Free Hamiltonian Vector Field]
The vector field defined by the local dynamics \eqref{eq:local_dyn} is divergence-free everywhere, which means:
    $$\nabla \cdot \Jkskew\nabla_{\mathbf{h}_v}H_{\mathcal{G}}(\mathbf{y}(t)) = 0 \text{, everywhere}$$
Hence, no sources or sinks can exist in the nonlinear dynamic.
\end{lemma}
\begin{proof}
Since the Hessian $\nabla^2H_{\mathcal{G}}(\mathbf{y}(t))$ is symmetric, it follows directly
    \begin{align*}
        \nabla \cdot \Jkskew\nabla_{\mathbf{h}_v}H_{\mathcal{G}}(\mathbf{y}(t)) 
        &=\sum_{i=1}^d{-\pdv[style-var=multipl]{H_{\mathcal{G}}(\mathbf{y}(t))}{q_{v}^{i},p_{v}^{i}}+\pdv[style-var=multipl]{H_{\mathcal{G}}(\mathbf{y}(t))}{p_{v}^{i},q_{v}^{i}}} = 0
    \end{align*}
\end{proof}

%\begin{lemma}[General Version of \cite{galimberti2023hamiltonian} Lemma 2]
%\label{lemma:flow_derivative_global}
%\end{lemma}
%\begin{proof}
%    We have $\dydt = f(\mathbf{y}(t))$ where $f(\mathbf{y}(t)) = \Jskew \nabla_{\mathbf{y}}H$. From Lemma \ref{lemma:flow_derivative_global} we can write that
%    \begin{equation}
%            \odv{}{t}\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)} = \left.\pdv{f}{\mathbf{y}}\right\rvert_{\mathbf{y}(T-t)}\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)} = \Jskew\left.\frac{\partial^2H}{\partial \mathbf{y}^2}\right\rvert_{\mathbf{y}(T-t)}\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)} = \Jskew S \pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)}
%    \end{equation}
%    with $S = S^{\top}$ as it is the Hessian of the Hamiltonian. Inspired by \cite{galimberti2023hamiltonian} we define $\Psi(T,T-t)=\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)}$. We know that $\Psi(T,T) = I$. Recalling that $\odv{\Psi(T,T-t)}{t} = \Jskew S \Psi$, if we take the derivative indicating $\Psi(T,T-t)$ simply as $\Psi$
%    \begin{equation}
%        \begin{split}
%            \odv{}{t}\left(\left[\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)} \right]^{\top}\Jskew \left[\pdv{\mathbf{y}(T)}{\mathbf{y}(T-t)}\right]\right) & = \dot{\Psi}^{\top} \Jskew \Psi + \Psi^{\top}\Jskew \dot{\Psi} = \\
%            & = \Psi^{\top} S^{\top} \Jskew^{\top} \Jskew \Psi + \Psi^{\top} \Jskew \Jskew S \Psi = \\
%            & = \Psi^{\top} S I \Psi + \Psi^{\top} (-I)S\Psi = 0
%        \end{split}
%    \end{equation}
%    which means that the objective $\Psi^{\top} \Jskew \Psi$ is constant $\Jskew$.
%\end{proof}
\begin{lemma}[Lemma 2, local version]\label{lemma:symplecticflow}
    We have that
    \begin{equation}
        \left[\pdv{\xk(T)}{\xk(T-t)}\right]^{\top} \Jskew_k \left[\pdv{\xk(T)}{\xk(T-t)}\right] = \Jskew_k
    \end{equation}
    where $\Jskew_k$ is the $2d \times 2d$ version of $\Jskew$ for $(p_k, q_k)$
\end{lemma}
Now we are ready to state our main result:
\begin{theorem}[Lower Bound, self-influence of the past]\label{theorem:continLowerBound}
    \begin{equation}
        \left\|\pdv{\xk(T)}{\xk(T-t)}\right\| \ge 1, \forall t \in [0,T].
    \end{equation}
    \begin{equation}
        \left\|\pdv{\xk(L)}{\xk(L-j)}\right\| \ge 1, \forall j = 0, \dots, L-1.
    \end{equation}
\end{theorem}
\begin{proof} Using Lemma \ref{lemma:symplecticflow} we can deduce for any sub-multiplicative norm $\|\cdot\|$ that:
\begin{equation*}
     \left\|\Jkskew \right\| = \left\| \left[\pdv{\xk(T)}{\xk(T-t)}\right]^{\top} \Jskew_k \left[\pdv{\xk(T)}{\xk(T-t)}\right] \right\| \le \left\| \pdv{\xk(T)}{\xk(T-t)}\right\|^2 \left\|\Jkskew\right\| 
\end{equation*}
\begin{equation*}
     \left\|\Jkskew \right\| = \left\| \left[\pdv{\mathbf{h}_v^{(L)}}{\mathbf{h}_v^{(L-j)}}\right]^{\top} \Jkskew \left[\pdv{\mathbf{h}_v^{(L)}}{\mathbf{h}_v^{(L-j)}}\right] \right\| \le \left\| \pdv{\mathbf{h}_v^{(L)}}{\mathbf{h}_v^{(L-j)}}\right\|^2 \left\|\Jkskew\right\| 
\end{equation*}
\end{proof}


\begin{theorem}[Upper Bound, Continuous]
    \begin{equation}
        \left\|\pdv{\xk(T)}{\xk(T-t)}\right\|_2 \le \sqrt{2d}\,\text{exp}(QT) \;\forall t\in[0,T]
    \end{equation}
    Where $Q = M\sqrt{2d}\,\|\mathbf{W}\|_2^2 + M\sqrt{2d}\,\text{max}_{i\in[n]}|\mathcal{N}_i|\|\mathbf{V}\|_2^2$ and $M$ satisfying $M > 0, |\sigma'(x)| \le M$, where $\sigma'(x)$ denotes any subderivative of $\sigma(x)$.
\end{theorem}

\begin{figure}
    \centering
    \includegraphics[width=0.325\textwidth]{figures/energy_10_SIE.png}
    \includegraphics[width=0.325\textwidth]{figures/self_gradients_toy_100.png}
    \includegraphics[width=0.325\textwidth]{figures/self_gradients_toy_1000.png}
    \caption{(left) Energy preservation in terms of difference to the initial state. (center) Log-Norms of 15 BSM matrices obtained through backpropagation on the Carbon-60 graph after 100 layers and 1000 layers (right).}\label{fig:grad_norms}
\end{figure}

\section{Related Work}
\cite{rusch2022graph,chamberlain2021grand,gutteridge2023drew}

Recalling the A-DGN model \citep{gravina2023adgn} which is designed in the light of the neural ODE perspective on ResNets and RNNs \citep{haber2017stable,chang2018antisymmetricrnn} to establish the critical criterion on the Jacobian creating a stable and non-dissipative system in the continuous domain. A known downside of this approach lies in translating this model into the discrete world since the forward Euler scheme requires a technical diffusion term to remain stable. Also, the key ingredient, an anti-symmetric parameterized weight matrix, limits the space of weight matrices that can be adjusted by backpropagation. Hence, it was already motivated by \cite{haber2017stable} to resort to Hamiltonian dynamics for ResNets to overcome the theoretical drawbacks of forward Euler discretization.

Using the Hamiltonian dynamics as building block for neural ODEs has led to neural networks tailored to simulate and predict observations of real physical systems \citep{sanchez2019hamiltonian,desai2021port}. In contrast to such works, this work follows the line of developing general-purpose architectures benefiting of the bias given by the Hamiltonian dynamics \citep{galimberti2023hamiltonian}. Just recently, fully auto-differentiated Hamiltonian models have been proposed that represent instances of graph neural networks \citep{KanZhaSon:C23,zhao2023adversarial}. These works are mainly concerned with the structure of the embedding manifold and its robustness to adversarial perturbations, leaving out theoretical properties regarding long-range interactions. To fill this gap, this work acknowledges the favorable properties of Hamiltonian dynamics and aims to derive and analyze explicit formulations for graph neural networks that exploit this dynamical system bias while being not restricted to simulate physical phenomena.

\section{Experimental Validation}
In order to analyze the contribution of different architectural choices to the performance of the overall model, the experimental setting of \cite{gravina2023adgn} is used. There, the tasks consist of predicting two node-level and one graph-level properties on synthetic graphs generated by different graph distributions. As the initial value for the node features, a Gaussian-normal distributed feature is fed into a linear layer to be projected into the latent space. The labels are determined by the specific task, all building up on the same graphs.

The first task is to predict the diameter of the graph, i.e., the maximum length of the shortest path in the entire graph. The second task is to predict the length of the single-source-shortest path (SSSP) to a randomly selected node in the graph. Here, the input features are extended with a binary value indicating if the node is the target node. The third task is considering the eccentricity of each node, i.e., the maximum length of all shortest paths started at the single node. In order to solve these tasks analytically, all shortest paths are required to be computed, hence long-range interactions at the length of the diameter must be computed by the graph neural network.
\subsection{Ablation on Graph Properties}
Downstream Task on p, q, (p,q)

Numerical Integration Scheme

Aggregation function as Vanilla, GCN

Port-Hamiltonian Architecture Search
Results in Table \ref{tab:graphproppred}
\begin{table}[ht]
    \renewcommand{\arraystretch}{1.1}
\centering
    \caption{Graph Property Prediction Baselines taken from \cite{gravina2023adgn}. Results given in the form of mean ${\pm\text{ std. dev}}$ after evaluation of 4 different seeds.}
    \label{tab:graphproppred}
    \begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccc}
\multirow{2}{*}{\textbf{Model}}&{\textbf{Diameter}} & {\textbf{SSSP}} & {\textbf{Eccentricity}} \\
&\newline{$\log_{10}\operatorname{MSE}$ $\downarrow$}&\newline{$\log_{10}\operatorname{MSE}$ $\downarrow$}&\newline{$\log_{10}\operatorname{MSE}$ $\downarrow$}\\\hline
\textbf{MPNNs} &&&\\
GCN &  0.7424  $\pm$ 0.0466  &  0.9499  $\pm$ 9.18$\cdot 10^{-5}$  &  0.8468  $\pm$ 0.0028  \\ 
GAT &  0.8221  $\pm$ 0.0752  &  0.6951  $\pm$ 0.1499  &  0.7909  $\pm$ 0.0222  \\ 
GraphSAGE &  0.8645  $\pm$ 0.0401  &  0.2863  $\pm$ 0.1843  &  0.7863  $\pm$ 0.0207  \\ 
GIN &  0.6131  $\pm$ 0.0990  &  -0.5408  $\pm$ 0.4193  &  0.9504  $\pm$ 0.0007  \\ 
GCNII &  0.5287  $\pm$ 0.0570  &  -1.1329  $\pm$ 0.0135  &  0.7640  $\pm$ 0.0355  \\ \hline
\textbf{DE-GNNs} &&&\\
DGC &  0.6028  $\pm$ 0.0050  &  -0.1483  $\pm$ 0.0231  &  0.8261  $\pm$ 0.0032  \\ 
GRAND &  0.6715  $\pm$ 0.0490  &  -0.0942  $\pm$ 0.3897  &  0.6602  $\pm$ 0.1393  \\ 
GraphCON  & 0.0964 $\pm$ 0.0620 & -1.3836 $\pm$ 0.0092& 0.6833 $\pm$ 0.0074\\
A-DGN\textsubscript{ws}(GCN) & 0.2271  $\pm$ 0.0804  &  -1.8288  $\pm$ 0.0607  &  0.7177  $\pm$ 0.0345\\
A-DGN\textsubscript{ws}(Vanilla) & -0.5455  $\pm$ 0.0328  &  -3.4020  $\pm$ 0.1372  &  0.3046  $\pm$ 0.1181\\ \hline
\textbf{Ours} & & &\\
H-DGN & -0.5473 $\pm$ 0.1074 & -3.0467 $\pm$ 0.1615 & -0.7248 $\pm$ 0.1068 \\
PH-DGN & -0.5473 $\pm$ 0.1074 & -4.2994 $\pm$ 0.0721 & -0.9348 $\pm$ 0.2097\\
\end{tabular}
\end{adjustbox}
\end{table}
\subsection{Long-Range Graph Benchmark}
Taken from the long-range graph benchmark of \cite{dwivedi2022long}, two graph tasks on peptides are of central focus to the experiment. Peptides are short chains of amino acids and hence, the nodes correspond to the non-hydrogen atoms while the edges represent the bonds between them. The first machine learning task is a multi-label graph classification further referred to as Peptides-func. Based on the biological functions, e.g., antibacterial, antiviral, or cell-cell communication, \cite{dwivedi2022long} collected 10 different classes.  Further, it is important to highlight that the labels are highly imbalanced: the biggest class has 62.7\% of all datapoints assigned, while the smallest is comprised of only 1.9\% of the data. Defined on the same splits, the second task is a multi-dimensional graph regression further referred to as Peptides-struct. Here, 3D properties of the peptides, e.g., inertia mass, inertia valence, length, or sphericity, need to be predicted.  \cite{tonshoff2023where} observed that 3-layer MLP with GELU activation and dropout (10\%) increases significantly the performance of the baseline models such as GCN. Results in Table \ref{tab:long_range}.
\begin{table}[ht]
\renewcommand*{\arraystretch}{1.2}
\centering
\caption{Baselines for Peptides-func (graph classification) and Peptides-struct (graph regression). Each experiment was run with 3-4 different seeds. Results taken from \cite{dwivedi2022long}, \cite{tonshoff2023where}, and \cite{gutteridge2023drew}.}\label{tab:long_range}
\begin{adjustbox}{max height=0.25\textheight} 
\begin{tabular}{lcc}
\multirow{2}{*}{\textbf{Model}} & 
\textbf{Peptides-func} & \textbf{Peptides-struct} \\
&  $\operatorname{AP}$ $\uparrow$ & $\operatorname{MAE}$ $\downarrow$ \\
\hline \textbf{MPNNs} & & \\
GCN &  0.5930 {  $\pm$ 0.0023}  &  0.3496 $\pm$ 0.0013  \\
GINE &  0.5498 {  $\pm$ 0.0079}  &  0.3547 $\pm$ 0.0045  \\
GCNII &  0.5543 {  $\pm$ 0.0078}  &  0.3471 $\pm$ 0.0010  \\
GatedGCN &  0.5864 {  $\pm$ 0.0077}  &  0.3420 $\pm$ 0.0013 \\
\hline \textbf{Transformer, Rewiring} & & \\
Transformer+LapPE &  0.6326 $\pm$ 0.0126 & 0.2529 $\pm$ 0.0016 \\
GraphGPS+LapPE & {${0.6535\pm  0.0041}$} & {${0.2500 \pm 0.0005 }$} \\
DRew-GCN+LapPE & 0.7150 $\pm$ 0.0044  & 0.2536 $\pm$ 0.0015\\
DRew-GCN & 0.6996 $\pm$ 0.0076 & 0.2781 $\pm$ 0.0028\\
\hline \textbf{DE-GNNs} & & \\
GRAND &  0.5789  $\pm$ 0.0062  &  0.3418 $\pm$ 0.0015  \\
GraphCON &  0.6022  $\pm$ 0.0068 & {${0.2778 \pm 0.0018 }$} \\
A-DGN &  0.5975 $\pm$ 0.0044  & ${0.2874  \pm 0.0021}$ \\
\hline \textbf{Re-Evaluated} & & \\
GCN+RWSE,LapPE &  0.6860 $\pm$ 0.0050 &  0.2460 $\pm$ 0.0007 \\
GINE+RWSE,LapPE &  0.6621 $\pm$ 0.0067  &  0.2473 $\pm$ 0.0017 \\
GCNII+RWSE,LapPE &  0.6765 $\pm$ 0.0047  &  0.2477 $\pm$ 0.0009  \\
GatedGCN+RWSE,LapPE &  0.6534 $\pm$ 0.0091  &  0.2509 $\pm$ 0.0014 \\
DRew-GCN+LapPE & 0.6945 $\pm$ 0.0021 & 0.2517 $\pm$ 0.0011\\
\hline \textbf{Ours} & & \\
H-DGN (1MLP) & 0.6652 $\pm$ 0.0051 & 0.3122 $\pm$ 0.0068\\
H-DGN (3MLP) & 0.7072 $\pm$ 0.0013 & 0.2554 $\pm$ 0.0004\\
PH-DGN (1MLP) & 0.5968 & 0.2825 $\pm$ 0.0048 \\
PH-DGN (3MLP) & - & 0.2486 $\pm$ 0.0016 \\
\end{tabular}
\end{adjustbox}
\end{table}

\section{Conclusion}
exploration of integrating an energy conservation bias into graph neural network architectures;
a neural network-parameterized Hamiltonian vector field was injected into the setup of graph-coupled neural ODEs;
symplectic integration led to an explicit layer-wise formulation representing an instance of message-passing neural networks; In line with Noether's theorem, the symmetries within the architecture give rise to the notion of energy preservation;
it could be shown that the Jacobian fulfills the critical criterion and gives rise to stable and non-dissipative behavior of the forward and backward pass. The key result is the lower bound on the backward sensitivity matrix which guarantees non-vanishing gradients within the continuous and discrete Hamiltonian graph neural network. At the same time, the Hamiltonian bias is causing the upper bound on the gradient to explode exponentially in terms of integration time and maximum size of the neighborhoods. 
Noting that the Hamiltonian dynamic marks a strong bias on the embedding manifold, tools taken from mechanical systems with friction and external control are integrated into the dynamics allowing eventually internal dampening of energy;

The model selection and ablation of the (port-)Hamiltonian graph neural networks demonstrated that new state-of-the-art scores can be reached on two out of three synthetic tasks;
Among classical message passing and differential equation-based architectures, the Hamiltonian dynamics lead to new state-of-the-art scores on classifying the biological function of the molecule, while performing on par with previous stable and non-dissipative graph neural networks on the second task. Especially, when considering tuned decoding architectures, overfitting is reduced and competitive scores are obtained that are on the level with rewiring approaches changing the underlying graph.
